Multi-view Content-aware Indexing for Long Document Retrieval

Long document question answering (DocQA) aims to answer questions from long documents over 10k words. They usually contain content structures such as sections, sub-sections, and paragraph demarcations. However, the indexing methods of long documents remain under-explored, while existing systems generally employ fixed-length chunking. As they do not consider content structures, the resultant chunks can exclude vital information or include irrelevant content. Motivated by this, we propose the Multi-view Content-aware indexing (MC-indexing) for more effective long DocQA via (i) segment structured document into content chunks, and (ii) represent each content chunk in raw-text, keywords, and summary views. We highlight that MC-indexing requires neither training nor fine-tuning. Having plug-and-play capability, it can be seamlessly integrated with any retrievers to boost their performance. Besides, we propose a long DocQA dataset that includes not only question-answer pair, but also document structure and answer scope. When compared to state-of-art chunking schemes, MC-indexing has significantly increased the recall by 42.8%, 30.0%, 23.9%, and 16.3% via top k= 1.5, 3, 5, and 10 respectively. These improved scores are the average of 8 widely used retrievers (2 sparse and 6 dense) via extensive experiments.

==> Table/ablation.tex <==
\begin{table}[tbp] 
\small
    \centering
    \resizebox{\linewidth}{!}{%
  \begin{tabular}{ll|cccc|c}
    \toprule
    \multicolumn{2}{c|}{\multirow{1}{*}{Chunk Scheme}}
    &  Top1 & Top 3 & Top5 & Top10 & ave $\Delta$ \\
    \midrule
    \parbox[t]{1mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{TF-IDF}}} 
    & \mname & & & & & - \\
    & - w/o raw text & & & & & \\
    &- w/o keyword & & & & & \\
    & - w/o summary & & & & & \\
    \midrule

    \parbox[t]{1mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{BM25}}} 
    & \mname & & & & & - \\
    & - w/o raw text & & & & & \\
    &- w/o keyword & & & & & \\
    & - w/o summary & & & & & \\
    \midrule

    \parbox[t]{1mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{DPR}}} 
    & \mname & & & & & - \\
    & - w/o raw text & & & & & \\
    &- w/o keyword & & & & & \\
    & - w/o summary & & & & & \\
    \midrule

    \parbox[t]{1mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{ColBERT}}} 
    & \mname & & & & & - \\
    & - w/o raw text & & & & & \\
    &- w/o keyword & & & & & \\
    & - w/o summary & & & & & \\
    \midrule

    \parbox[t]{1mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Contriever}}} 
    & \mname & & & & & - \\
    & - w/o raw text & & & & & \\
    &- w/o keyword & & & & & \\
    & - w/o summary & & & & & \\
    \midrule

    \parbox[t]{1mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{E5}}} 
    & \mname & & & & & - \\
    & - w/o raw text & & & & & \\
    &- w/o keyword & & & & & \\
    & - w/o summary & & & & & \\
    \midrule

    \parbox[t]{1mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{BGE}}} 
    & \mname & & & & & - \\
    & - w/o raw text & & & & & \\
    &- w/o keyword & & & & & \\
    & - w/o summary & & & & & \\
    \midrule

    \parbox[t]{1mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{GTE}}} 
    & \mname & & & & & - \\
    & - w/o raw text & & & & & \\
    &- w/o keyword & & & & & \\
    & - w/o summary & & & & & \\
    % \midrule
    
  \bottomrule
  \end{tabular}
  }
\caption{Ablation study for WikiWeb2M and NQ, $\Delta$ refers to the average decrease of top 1, 3, 5, and 10.}
\label{tab:ablation}
\end{table}


